Indoor Smartphone SLAM with Learned Echoic Location Features

Indoor self-localization is a highly demanded system function for smartphones. The current solutions based on inertial, radio frequency, and geomagnetic sensing may have degraded performance when their limiting factors take effect. In this paper, we present a new indoor simultaneous localization and mapping (SLAM) system that utilizes the smartphone's built-in audio hardware and inertial measurement unit (IMU). Our system uses a smartphone's loudspeaker to emit near-inaudible chirps and then the microphone to record the acoustic echoes from the indoor environment. Our profiling measurements show that the echoes carry location information with sub-meter granularity. To enable SLAM, we apply contrastive learning to construct an echoic location feature (ELF) extractor, such that the loop closures on the smartphone's trajectory can be accurately detected from the associated ELF trace. The detection results effectively regulate the IMU-based trajectory reconstruction. Extensive experiments show that our ELF-based SLAM achieves median localization errors of $0.1\,\text{m}$, $0.53\,\text{m}$, and $0.4\,\text{m}$ on the reconstructed trajectories in a living room, an office, and a shopping mall, and outperforms the Wi-Fi and geomagnetic SLAM systems.

==> Makefile <==
DOC=main

dvi:
	if [ ! -f dvimode ] ; \
	then \
		echo "Entering dvimode" ; \
		echo "" > dvimode ; \
		sed -i '/\RequirePackage\[prologue\]{xcolor}/c\\\RequirePackage{xcolor}' acmart.cls; \
	fi;
	latex -src-specials -halt-on-error main
	#pdflatex -synctex=1 -src-specials -interaction=nonstopmode main

bib:
	bibtex main

pdf:
	if [ -f dvimode ] ; \
	then \
		echo "Exiting dvimode" ; \
		rm -f dvimode ; \
		sed -i '/\RequirePackage{xcolor}/c\\\RequirePackage\[prologue\]{xcolor}' acmart.cls; \
	fi;
	latex main
	dvips main.dvi
	ps2pdf main.ps
	#pdflatex main

drop:
	unison dropbox ~/research/SonarSLAM/writeup ~/Dropbox/echoLoc

all:
	pdflatex $(DOC).tex
	bibtex $(DOC)
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex

upload: 
	unison . ../Elf-SLAM/

==> Makefile_backup <==
DOC=main

dvi:
	if [ ! -f dvimode ] ; \
	then \
		echo "Entering dvimode" ; \
		echo "" > dvimode ; \
		sed -i '/\RequirePackage\[prologue\]{xcolor}/c\\\RequirePackage{xcolor}' acmart.cls; \
	fi;
	latex -src-specials -halt-on-error main
	#pdflatex -synctex=1 -src-specials -interaction=nonstopmode main

bib:
	bibtex main

pdf:
	if [ -f dvimode ] ; \
	then \
		echo "Exiting dvimode" ; \
		rm -f dvimode ; \
		sed -i '/\RequirePackage{xcolor}/c\\\RequirePackage\[prologue\]{xcolor}' acmart.cls; \
	fi;
	latex main
	dvips main.dvi
	ps2pdf main.ps
	#pdflatex main

drop:
	unison dropbox ~/research/SonarSLAM/writeup ~/Dropbox/echoLoc

all:
	pdflatex $(DOC).tex
	bibtex $(DOC)
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex

upload: 
	unison . ../../echoLoc/

==> background.tex <==

\section{Background}

\subsection{Challenges of Acoustic Sensing}

An active sound travels inside an indoor space will interacts with the environment in a way that reflections, absorbtions and diffractions are intrigued together prior arriving to the receiver. Room impulse response (RIR) is often measured to describe such acoustic phenomenon of a room \cite{di2021dechorate}. RIR is widely used in applications like speech enhancement, room geometry estimation, mcirophone calibration, etc. In practice, the RIR is measured by exciting a short impulse signal inside a room then use a microphone to record the signals at different locations. In principle, the RIR reflects the sound source interactions with rooms and carries the information like sound source location and receiver location. Different locations inside a room should exhibit different RIRs. It is possible to exploit the property of RIRs to infer the location of a receiver inside a room. 



% {\red challenges: (1) training data volume; (2) feature effectiveness}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> contrastive.tex <==


\subsection{System Overview}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> indoor_location.tex <==
\subsection{Large-Scale Indoor Localization using acoustic fingerprints}
\label{sec:indoor-loc}

We have demonstrated the spatial distinctness and temporal stability of acoustic features collected by a smartphone. Therefore, a fingerprinting- based approach can potenitally be exploited for localization using a smartphone. We show that acoustic features can be used for high granularity localization in an indoor space.

% We treat obtained echo spectrograms as 1-channel images and train a CNN for location classification. We adopt ResNet-18 architecture and customize the first layer to allow the a-channel spectrogram images as input. We implement the ResNet-18 using Pytorch.
\subsubsection{Data collection and model design}

  \begin{figure}
	\begin{subfigure}[t]{.55\columnwidth}
	  \includegraphics[width=\columnwidth]{eps/ncs_v1}%{eps/conventional-da}
	  \caption{Laboratory office floor plan}
	  \label{fig:ncs-layout}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{.4\columnwidth}
	  \includegraphics[width=\columnwidth]{eps/cdf_1vote}
	  \caption{Localization error CDF}
	  \label{fig:ncs-cdf}
	\end{subfigure}
	%\vspace{-0.5em}
	\caption{Lab space and evaluation result.}
	\label{fig:ncs-eval}
	%\vspace{-2em}
  \end{figure}

We conduct the experiment in a real laboratory office. The floor plan is shown in Fig.~\ref{fig:ncs-layout}, it is a $16 {\text m} \times 28 {\text m}$ space consists of a large cubicle area, a social lobby and multiple meeting rooms. We use a smartphone to collect 100 locations' fingerprints in the laboratory. The red squares in Fig.~\ref{fig:ncs-layout} mark the locations where fingerprints are collected from. The fingerprinted locations cover the commonly visited locations in the lab: cubicle seat tables, demo rooms, social discussion lobby and the meeting room.

For data collection, A surveyor holds a smartphone at chest level to visit each location for data collection. Measurement studies shows that the acoustic features are sensitive to the orientation and user height. We therefore ask the surveyor to move around the phone at each location to have a better coverage of phone positions. We collect {\red 1500 fingerprints as training data and 200 fingerprints} as test data for each location, and record the corresponding coordinates and use as the label. 

To address the training data scarcity of acoustic echoes and avoid extensive data collection by humans. We propose to augment the training data for CL by leveraging on the data produced by simulation tools. Note that a room's acoustic response is determined by various factors including its shape, wall materials, objects that occupy the room, material absorption and reflection rate, etc. The existing simulation tools are not yet able to generate accurate acoustic response to mimic a real room. We demonstrate this using an example. We employ pyroomacoustic \cite{scheibler2018pyroomacoustics} to construct a room with similar size to the demo room as shown in Fig.~\ref{fig:demo-room}. We use a 0.5 energy absorption for all walls. In simulation, we place a omni-diectional sound source at the center of the room and plays the deisigned logarithmic chirp. In addition, we mimic a smartphone recording by placing a microphone at 15$cm$ apart from the sound source to record the signal. We follow the same procedures in \sect\ref{subsec:chirp-design} to extract the spectrogram of the echo and compare it with a real spectrogram obtain from the same location in the real room. Fig.~\ref{fig:real-sim}a,~\ref{fig:real-sim}b show a comparison of simulated and real spectrogram. It is obvisously that the spectrograms are different in terms of the frequency energy distribution is time domain. 
  
Despite the acoustic features generated by simulation tool are different from a real room, the simualated acoustic features can be used for the purpose of contrastive feature representation learning. Fig.~\ref{fig:real-sim}b,~\ref{fig:real-sim}c show the spectrograms generated using $pyroomacoustic$ at two locations with 0.5$m$ apart. The generated features are spatially distinct, indicating that we can use the simulation to generate data for to augment the training dataset.  

We extract echo' spectrogram feature and train a DNN to evaluate the localization performance. Specifically, we treat obtained echo spectrogram as a 1-channel image and deploy the CNN for location classification. We adopt the ResNet-18 architecture and customize the first layer to allow the a-channel spectrogram images as input. The model is implemented using Pytorch. Fig.~\ref{fig:ncs-cdf} shows the cumulative distribution function (CDF) of the localization errors in meters. It shows that fingerprinting-based acoustic localization achieves a median error of 0.5\text{m}, and 90\% tile localization error is 1\text{m}.

\subsubsection{Performance evaluation}
\begin{figure}
	\begin{subfigure}[t]{.45\columnwidth}
	  \includegraphics[width=\columnwidth]{eps/cdnn_acc_vs_data_volumn}%{eps/conventional-da}
	  \caption{Model accuracy vs data volumn}
	  \label{fig:dnn-acc}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{.45\columnwidth}
	  \includegraphics[width=\columnwidth]{eps/cdnn_acc_vs_data_volumn}
	  \caption{TBA}
	  \label{fig:tba}
	\end{subfigure}
	%\vspace{-0.5em}
	\caption{TBA.}
	% \label{fig:tba}
	%\vspace{-2em}
  \end{figure}

DNN-based localization requires substantial training data, albeit achieves sub-meter localization errors. We plot {\red fig xx} to characterise the DNN's performance against the volumn of training data. Horizontal axis represents the training data available for each location, vertical axis represent the DNN localization accuracy on test dataset. It's expected that DNN's performance increases with more training data available for each class. We observe that DNN's performance saturated when number of training data in each class larger than 1500, representing 5 hours' training data collection time. Although it is one-time effort, long training data collection time still impede the applicability of DNN-based approach. 

The research question is, how can we reduce the training data collection effort whereas maintains the performance of DNN for localization?


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> intro_backup.tex <==
\section{Introduction}
\label{sec:intro}
Due to proliferation of smartphones nowdays, the smartphone based positioning attracts lots of interest and is a key enabler for location-based services. Unlike in outdoor environment that a smartphone can be positioned via GPS, accuract smartphone indoor positioning remain challenging due to: 1) the blockage of satellite signal make GPS service unavailable within the building. 2) complex and dynamic indoor environment renders indoor positioning challenging, 3) miniaturized smartphone sensors design leads to inaccuracte and noisy sensors readout, 4) heterogeneous smartphone sensors further halts the generability of tailored positioning algorithm.

Smartphone based indoor positioning exploits smartphone embedded sensors for smart sensing. They assume the availability of target signal within a room, e.g. WIFI, bluetooth low energy (BLE), FM radio and magnetic signal. They use smartphone embedded sensors to probe received signal strenth (RSS) or channel state information (CSI). Smartphone position can be inferred through signal propagation model or radio map reconstruction. 

WIFI based localization exploits RSSI or CSI information received at mobile device for localization. Traditional approaches uses AoA, ToF of received signal for localization. Recent research exploits state-of-the-art deep neural network (DNN) that converts localization problem to image translation problem. In general, wifi-based indoor localization can achieve sub-meter accuracy. However, received wifi signal usually affected by device orientation, signal reflection/attenuation, and even from device heterogeneity. The complicated indoor environment often poses multi-path reflection and non-line of sight problem. Fingerprinting based approach generally require significant amount of effort for radio map construction, DLoc (MobiCom20) \cite{ayyalasomayajula2020deep} designed a robot to collect fingerprinting data.
BLE based indoor localization requires beacons to pre-install within the area of interest. Mobile devices receives the signals from beacons and use AoA or ToF for multilateration. BLE-based approach can achieve sub-meter accuracy. However, it requires additional beacon installation, which stems its popularity. FM based localization assumes the full coverage of FM radio within the indoor area. It exploit RSS received on mobile device to construct radio map prior localization. The location of unknown signal is calculated by nearest-neighbor algorithm. FM based approach can achieve meter-level error and it does not require additional infrastructure. While this approach requires the coverage of FM radio and intensive fingerprinting data collection is unavoidable.
Acoustic localization, which exploits the acoustic system embedded on mobile device for ranging receives more interest recently. Acoustic sensing uses its speaker to play pre-defined chirps within a room and uses its microphone to capture the reverberation. Thre received reverberation inherently represents the interaction between acoustic signal and enclosed area, one can exloit the reverberation for smart sensing. Ecotag uses a smartphone to playback a chirp to discriminate different location tagging. Howerver, this approach is different from localization task as Ecotag can only remember the known locations. Roomsense extract the MFCC features from acoustic echoes and apply fingerprining approach for localization. However, they only achieve 3 meter localization error, which is not applicable for indoor localization. ALPS uses BLE and untrasound for localization. However,their approach requires additional beacon setup at LOS area.

For general indoor localization application, there is a trade-off between accuracy and computing complexity. For general usage like patient tracking, customer location awareness application, we argue that sub-meter to meter level accuracy is suffice. In this paper, we present {\red XXX} which exploit mobile device acoustic system for indoor localization. Specifically, our system leverages on the state-of-the-art machine learning model to model acoustic reverberation within a room. When a user enters a new environment, a minimum effort of collecting few fingerprinting data is sufficient for model transfer. Additional, this system does not require external anchors installation but only requires {\red the room dimension information which is readily available.}

technology have been studied in last few decades,
inaccurate in indoor condition due to block of signals. 

Unlike outdoor localizations that a smartphone can be located via GPS, indoor localizations that is key enabler for location-based services. For example, hospital can track 
The remainder of this paper is organized as follows.
\sect\ref{sec:conclude} concludes this paper.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> measurement-old.tex <==
\section{Measurement Study}
\label{sec:measure}

{\red this section provides the basic understanding of the echoic location feature}
% We use a smartphone's speaker to emit probing chirps in a room and record the room's echo using the smartphone's microphone. 
% We firstly present the probing chirp design and acoustic feature selection. Then we show that the acoustic features have the properties for localization.

% \subsection{Probing Chirp Design}
% \label{subsec:chirp-design}
% Existing research utilizes smartphone's built-in acoustic system to emit specifically designed audio signals and collect environment's responses for different applications.
% EchoTag \cite{tung2015echotag} uses the phone's speaker to play a series of linear sweeping chirps ranging from 11kHz to 20kHz and analyses the microphone-collected room's echos for indoor location tagging. The audible frequency range of the emitted chirps cause inevitable annoyance to human users. Moreover, it takes more than 2 seconds to infer the tag of a location each time because for each location, the speaker needs to emit 16 single-tone chirps sequentially with an interval of 0.1 second.
% DeepRoom \cite{song2018deep} employs a single-tone chirp at the inaudible frequency of 20kHz for room-level indoor localization. The emitted chirp is merely $2\,\text{ms}$. Thus, the room's responses to this simple and short audio signal only carry limited information about sensed environment.

\subsection{Experiment Setup}

\subsubsection{Probe signal design and siganl processing}
\label{subsec:chirp-design}

\begin{figure}
	\includegraphics[width=\columnwidth]{eps/prob_chirp_box}
	\caption{Probe signal design.}
	\label{fig:probe-chirp}
\end{figure}

The design of the probing signal is crucial in active acoustic sensing. The most commonly used signals include single tone, frequency hopping spectrum spread (FHSS), and chirp \cite{cai2022ubiquitous}. Single tone benefits from its low complexity and high sensitivity to doppler shift. Thus, it is widely adopted in localization \cite{song2018deep}, tracking \cite{yun2015turning}, and gesture recognition \cite{gupta2012soundwave}. However, we consider using multi-frequency signals because we aim to design the probe signal such that the echos can carry richer information about the sensed environment and achieve fine-grained spatial distinctness. FHSS signal rapidly changes the frequency of the carrier occupying a wide spectral band. Correlating FHSS signal achieves sharper peaks and smaller sidelobes, which results in high accuracy tracking \cite{yun2017strata}. However, the highly sensitive FHSS signal is easily affected by noises and is more suitable for short-range sensing. Thus, we employ chirp signal that carries richer information and is suitable for long-range sensing \cite{cai2022ubiquitous}. The frequency of a chirp increases or decreases with time. The commodity smartphones usually support audio sampling rates of 44.1 kHz or 48 kHz. Thus, according to the Nyquist theorem, the smartphone acoustic system can send and receive acoustic signals with frequency up to 24 kHz. To eliminate the interferences from man-made sounds and background noises, the probe signal should occupy an inaudible or nearly inaudible frequency range. The theoretical frequency range of human detectable sounds is from 20 Hz to 20 kHz \cite{audiblespectrum}. Since human can lose high frequency sensitivity as they mature, the upper bound in average adults is usually 15-17 kHz. When the frequency is higher than 20 kHz, the signals emitted from smartphone's speaker suffer from drastic distortions \cite{song2018deep}, which is possibly due to hardware imperfection. Therefore, as shown in Fig.~\ref{fig:probe-chirp}, we implement the logarithmic chirp ranging from 15 kHz to 20 kHz with a chirp duration of $10\,\text{ms}$ to be our probe signal. We aim to employ a wider frequency band to capture finer-grained spatial features, while making the probe signal nearly inaudible. We emit this probe chirp and collect echos in different indoor locations using the smartphone's built-in speaker and microphone.


% We investigate the hardware specifications of commercial smartphones' audio systems to obtain the optimal settings for frequency range $f_{1}$, $f_{2}$ and time duration $T$. A smartphone's audio system usually supports {\text 44.1kHz} sampling rate, the theoretical upper bound of the frequency can be sensed is at 22kHz according to the Nyquist theorem. However, the quality of the sensed audio signals drops significantly when the frequency is higher than 20kHz due to the imperfection of smartphone hardwares \cite{song2018deep}. Therefore, we set upper bound frequency $f_{2}$ at 20kHz to maintain the quality of the sensed audio signal. We choose a logarithmic chirp with {\text 5kHz} frequency band to ensure a rich information will be contained in the echo, thus the lower frequency of the signal is {\text 15kHz}. A human generally can hear the sound up to {\text 18kHz}, our signal lies in {\em near-inaudible} range of human ear. We conducted experiments on a few commercial smartphones to explore the shortest possible time to generate the designed sweeping signal at he given band. The result shows that $10\,\text{ms}$ is the shortest time to generate a sweeping signal from {\text 15kHz} to {\text 20kHz}. To summarize, we design a short sweeping chirp that lies in near-inaudible range as our probing chirp for location sensing.

\begin{figure}
	\includegraphics[width=\columnwidth]{eps/chirp_process_box}
	\caption{Echos in response to probe signal received by the phone's microphone.}
	\label{fig:received}
\end{figure}

\begin{figure}
	\includegraphics[width=\columnwidth]{eps/specs_box}
	\caption{Spectrograms extracted from three indoor locations.}
	\label{fig:specs}
\end{figure}

% $\blacksquare${\bf Acoustic Signal Processing: }
We extract the location spectrogram from the received echos. As shown in Fig.~\ref{fig:received}, we discard the direct path from phone's loudspeaker to its microphone and keep the subsequent 2400 samples to compute the spectrogram. From Fig.~\ref{fig:received}, if we compute the correlation between the received echos and the template probe signal, we can see multiple wave packets. This suggests that the smartphone's acoustic system is able to emit and receive the probe signal. Next, we apply a high-pass filter with a cut-off frequency of $15\,\text{kHz}$ to the 2400-sample echos. Then, we employ short-time Fourier transform (STFT) together with Hanning window that has length of 96 sample points and overlapping of 48 sample points to obtain the spectrogram of the echos. We only keep the frequency bins of 15-20 kHz. The resulting spectrogram has size of $12 \times 48$. Fig.~\ref{fig:specs} shows the spectrogram extracted from three different indoor locations. We can perceive the difference in these features, indicating that our probe signal has the capability to distinguish different indoor locations. 
% The received the sound siganl from microphone contains the direct path that is played back from the smartphone speaker followed by the reverberated echeos. We discard the signals due to the direct path since it does not contains useful information for location sensing and keep the subsequent 2400-samples as the echo feature {\red (need justify why 2400)}. Second, a high-pass filter with a cut-off frequency of $15\,\text{kHz}$ is applied to the echoes. This step can effectively remove the contamination of background noises as most of them lie in lower frequencies. Third, short-time Fourier transform (STFT) is applied on the signal to calculate the power spectral density (PSD). Specifically, we slide a 96-point Hann window with 48 points of overlap on echo data, resulting a $49 \times 48$ spectrogram. We further discard the frequency bins below $15\,\text{kHz}$, yielding a $12 \times 48$ image as the final feature. Fig. ~\ref{fig:echo_f}d shows the spectrogram plot of the echo feature. We can see the expected energy distribution from 15kHz to 20kHz, indicating that the smartphone's microphone correctly captures reflections from the surrounding space from the played chirp. The other observation is that the energy at the later range in the spectrogram is smaller, meaning that the energy of echoes decays fast. % Note that we only keep the magnitude of each bin and discard the phase information.
% An instance of sensing signal to be played from the smartphone is shown in Fig. ~\ref{fig:echo_f}a. The signal consists of 500-samples (10ms) designed chirp followed by a 4000-sample silence. Similar to \cite{tung2015echotag}, the silence inserted in between the chirps is used to separate chirps for preventing the interference of chirps and allowing the echoes from the precedent chirp to be recorded by smartphone's microphone. Fig. ~\ref{fig:echo_f}b shows an instance of recorded echo by smartphone microphone. The recorded signal contains the large amplitude chirps, which is corresponding to the direct signal recorded from the phone's speaker. The subsequent signals with lower amplitude are the echoes due to the room's reflection. Fig. ~\ref{fig:echo_f}c is the spectrogram representation of Fig. ~\ref{fig:echo_f}b of logarithmic chirp, we can see that smartphone plays the expected chirp in 15kHz to 20kHz range. % The spectrogram of echoes is not visually observable due to the small energy compared to the direct path signal. 

\subsubsection{Experiment environment and data collection}

% \begin{figure}
% 	\begin{subfigure}[t]{.55\columnwidth}
% 	  \includegraphics[width=\columnwidth]{eps/ncs_v2}%{eps/conventional-da}
% 	  \caption{Floor plan of the university lab. Echos are collected from the locations illustrated by red squares.}
% 	  \label{fig:ncs-layout}
% 	\end{subfigure}
%   %   \hfill
%   %   \begin{subfigure}[t]{.4\columnwidth}
%   % 	\includegraphics[width=\columnwidth]{eps/cdf_ncs127_1vote}
%   % 	\caption{Localization error CDF}
%   % 	\label{fig:ncs-cdf}
%   %   \end{subfigure}
% 	%\vspace{-0.5em}
% 	\caption{Lab space and evaluation result.}
% 	\label{fig:ncs-eval}
% 	%\vspace{-2em}
% \end{figure}

\begin{figure}
	\centering
	\includegraphics[width=.75\columnwidth]{eps/ncs_v2}%{eps/conventional-da}
	\caption{Floor plan of a university lab.}
	\label{fig:ncs-layout}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=0.78\columnwidth]{eps/measure_log_chirp_tsne2d}
		\caption{Chirp.}
		\label{fig:tsne-log}
	\end{subfigure}
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=0.78\columnwidth]{eps/measure_20khz_chirp_tsne2d}
		\caption{Single tone.}
		\label{fig:tsne-20khz}
	\end{subfigure}
	\caption{t-SNE of the spectrograms on five locations in a demo room.}
	\label{fig:tsne-result}
\end{figure}

The experiments for our measurement study are conducted in a university lab environment as shown in Fig.~\ref{fig:ncs-layout}. The lab size is $16 {\text m} \times 28 {\text m}$.  
% consists of a main lab space, two demo rooms, a social lobby and two meeting rooms with slightly different sizes. 
We use a {\red xxx smartphone} to emit probe chirps with its speaker and receive echos with its microphone in 127 locations illustrated in red squares. Then, we extract spectrograms from the received echos, as described in \sect\ref{subsec:chirp-design}. 
% The collected fingerprints vary on spatial distances (SD): the SD for meeting room table is around $25 {\text cm}$, the SD for meeting room seat is around $50 {\text cm}$, the SD for demo room table seat is around $100 {\text cm}$, the SD for lab space table seat is around $150 {\text cm}$.   
For each location, we collect 1,700 spectrograms.
% we collect 1,500 fingerprints as training data and 200 fingerprints as test data, and record the corresponding coordinates as the true label. 

% \subsection{Experiment Results}

% As summarized in Table.~\ref{tab:chirp-design-acoustic-sensing}, the probing signal designs of existing acoustic localization applications either sweep a wide frequency band for a long time duration or carry only limited information due to the short-time and simplicity of the probing signal. To address these limitations, we aim to design a signal that meets the following three requirements. 
% First, the chirp should be {\bf complex} to carry rich information about the sensed environment. Second, the chirp is desired to fall in the {\bf near-inaudible} frequency ranges of human to eliminate annoyance. Last but not least, the chirp needs to be {\bf short} to reduce the sensing time of the end-user {\red need to explain why needs to be short}. 
% To fulfill these three requirements, we propose to use a frequency-varying logarithmic chirp as described in eq.~\ref{eq:log_chirp} \cite{farina2000simultaneous}. 
% \begin{equation}
%   x[i] = \sin \left( \frac{2\pi f_{1} T}{\ln \left( \frac{f_{2}}{f_{1}} \right)} \cdot \left( e^{\frac{i}{f_{s} T} \cdot \ln \left( \frac{f_{2}}{f_{1}} \right)} - 1 \right) \right),
%   \label{eq:log_chirp}
% \end{equation}
% Where $f_{1}$ and $f_{2}$ are the lower and higher bound of the chirp frequency in Hz, $f_{s}$ is the sampling rate and $T$ is the chirp duration in second.
% The sweeping logarithmic audio signal covers multiple frequencies % that lies in the near-inaudible hearing range of human, 
% thus will enrich the information carried by the echos. % and reduce the annoyance caused during the probing. 

\begin{comment}
Prior works \cite{tung2015echotag,song2018deep} utilize the smartphone's acoustic system to play the specially designed acoustic signals to probe a room's acoustic response for indoor location tagging or room-level recognition. The existing commercial smartphones support 44.1kHz of sampling rate for recording. By Nyquist theorem, the smartphone can sense the signal with frequency up to 22kHz. EchoTag \cite{tung2015echotag} designs a linear sweeping chirp in the range of 11kHz to 20kHz, with a step size of 2750Hz. The sweeping chirp designed by EchoTag consists of multiple frequencies, thus it is able to sense the room's reflections that characterizing different frequencies. However, the lowest frequency used by EchoTag is 11kHz, it is inevitable to cause the annoyance to a human user as the chirp is hearable by the human. EchoTag tries to ease the annoyance by tuning down the chirp volume to 5\% of the maximum. However, a low volume of sweeping chirp will have a low signal-to-noise ratio (SNR), thus limiting its sensing range. In addition, the total sensing time of a full chirp is near 2-3 seconds, as the sweeping chirp consists of 16 single-tone chirps and each is separated by a 0.1 second waiting time. 
On the other hand, DeepRoom \cite{song2018deep} employs an inaudible single-tone chirp for sensing, the frequency used is 20kHz. Compared to EchoTag, the chirp designed by DeepRoom is inaudible to the human thus introduces little annoyance. The sensing time is merely 2{\text ms}, which far shorter than EchoTag. However, the acoustic feature probed by DeepRoom contains less information compared to EchoTag as only a single frequency is used. In what follows, we show that the acoustic feature extracted from a single-tone chirp is not optimal for location discrimination.

Therefore, the ideal probing chirp for indoor location discrimination should fulfill the three requirements: {\bf enrichment},{\bf inaudibility} and {\bf quickness}. {\bf Enrichment:} the signal should contain multiple frequencies to include the room's reflections characterized by different frequencies. {\bf Inaudibility}, the probing chirp is preferred in the inaudible range of human hearing, thus the signal will cause no/little annoyance to a user. {\bf Quickness}, a short probing time is desired from an end-user. A short sensing time renders the signal robust to the ambient noises and more reliable data can be collected in the given period of time.
EchoTag fulfills the {\bf enrichment} requirement, whereas fails the {\bf inaudibility} and {\bf quickness}. DeepRoom meets the {\bf inaudibility} and {\bf quickness} but fails {\bf enrichment}.

To meet all requirements for indoor location probing, we propose a varying-frequency sine sweep chirp that ranges from 15kHz to 20kHz. There are two consideration for the selected frequency range: first, unlike EchoTag that sweeping from 11kHz, 15kHz is lies in near-inaudible range of human hearing, thus causes little annoyance. Second, we set the upper bound of signal to 20kHz by considering the imperfection of smartphone hardware. As shown in \cite{song2018deep}, although the theoretical maximum frequency can be sensed is 22kHz at a sampling rate of 44.1kHz, a smartphone has a poor performance to record frequency higher than 20kHz due to hardware imperfection \cite{song2018deep}. The used 15kHz to 20kHz sweeping chirp meet the requirements of {\bf enrichment},{\bf inaudibility}. There are two commonly used approaches to generate varying-frequency chirp: linear sweep and logarithmic sweep. The linear sweep approach generates a chirp that has equally distributed energy within the frequency range. Unlike EchoTag that uses a step size of 2750Hz, thus its sweeping chirp only contains four valid frequencies, we gradually increase the frequency from 15kHz to 20kHz in the given time, thus our designed signal contains more frequencies. We adopt the approach in \cite{farina2000simultaneous} to generate a logarithmic chirp.
To meet the {\bf quickness} requirement, we use a smartphone to conduct experiments to evaluate the shortest chirp a phone can generate. We valided on a Google Pixel-4 phone and found that it is able to generate logarithmic chirp from 15kHz to 20kHz in time as short as 10{\text ms}.
\end{comment}
% For monotone sine chirp, we use a 10-ms single tone chirp of 20kHz similar to \cite{song2018deep}.
% We use an Android smartphone to playback the probing chirps and record the room's reverberation.

\subsection{Spatial Distinctness of echoes}

% 20_paper_plot_measurement_chirp_type
% \begin{figure}
% 	% \vspace{1em}
% 	% \subcaptionbox{Demo room layout\label{fig:demo-room}}{\includegraphics[width=\columnwidth]{eps/ncs_demo_room_layout}}\hfill%
% 	\subcaptionbox{Chirp\label{fig:tsne-log}}{\includegraphics[width=0.48\columnwidth]{eps/measure_log_chirp_tsne2d}}\hfill%
% 	% \subcaptionbox{Linear chirp\label{fig:tsne-linear}}{\includegraphics[width=0.33\columnwidth]{eps/measure_linear_chirp}}\hfill%
% 	\subcaptionbox{Single tone\label{fig:tsne-20khz}}{\includegraphics[width=0.48\columnwidth]{eps/measure_20khz_chirp_tsne2d}}\hfill%

% 	\caption{t-SNE features of the received echos on five locations in response to chirp and single tone signals.}
% 	\label{fig:tsne-result}
% 	%\vspace{-1em}
% \end{figure}

In this section, we investigate the spatial distinctness of the received echos. We collect spectrograms from five locations in the demo room of the lab. Each locations are about 1m apart from each other. We then apply T-distributed stochastic neighbor embedding (t-SNE) to reduce the dimension of the spectrograms and visualize them in 2D space. The results are shown in Fig.~\ref{fig:tsne-result}. It can be observed that the t-SNE features of the echo's spectrograms corresponding to different locations are well separated in 2D space. In particular, the spectrograms of the chirp signal exhibit better location distinguishability than those of the single tone signal. This preliminary experiment implies that our probe signal can achieve fine-grained and spatially distinct echos.

In the following experiments, we use the indoor localization task to systematically evaluate the spatial distinctness of the echos. Specifically, for each of the 127 locations where we collect echos from, we divide the spectrograms into 1,500 training samples and 200 test samples. The ground truth labels for the samples correspond to the coordinates of the locations. Then, we train the ResNet-18 model with the training data samples for location classification. The localization performance in terms of resolution, scalability, and stability is evaluated using the test samples.

% We extract the echo's spectrogram feature and train a DNN to evaluate the localization performance. Specifically, we treat obtained echo spectrogram as a 1-channel image and deploy the CNN for location classification. We adopt the ResNet-18 architecture and customize the first layer to allow a one-channel spectrogram image as input. The model is implemented using Pytorch. % Fig.~\ref{fig:ncs-cdf} shows the cumulative distribution function (CDF) of the localization errors in meters. It shows that fingerprinting-based acoustic localization achieves a median error of $0.58 \text{m}$, and 90\% tile localization error is $1 \text{m}$.


% We conduct a set of measurements to investigate whether the recorded acoustic features at different locations in an indoor space are distinct, and what type of chirp yields the best performance. 

% {\bf Spatial Distinctness of Different Chirps:} We evaluate the spatial distinctness of different chirps in a demo room of about 60 $m^2$. Fig.~\ref{fig:demo-room} is the floor plan of the demo room, we record the acoustic features at the red-square spots labeled from 0 to 4, each is 1$m$ apart. We play and record 10 echoes for each type of chirp at each spot. We extract the echo's spectrogram for feature analysis. We use T-distributed stochastic neighbor embedding (t-SNE) to reduce the dimension of the spectrogram and visualize them in 2D space. Fig.~\ref{fig:tsne-log},~\ref{fig:tsne-linear} and ~\ref{fig:tsne-20khz} show the visualization results of three chirps. We can see that features extracted from linear or logarithm sweeping chirps at different spots are distinct and well separated, whereas the features from monotone chirp is less effectively separated. Based on this observation, we conclude that linear and logarithmic sweeping chirps are more suitable for room acoustic sensing. We use logarithmic sweeping chirp for the remaining experiments in this paper.

% jiebi_code/21_paper_plot_measure_height_2
% jiebi_code/22_paper_plot_measure_orient_2
% jiebi_code/22_paper_plot_measure_time
\begin{figure}
	% \vspace{1em}
	\subcaptionbox{Height effect (cm)\label{fig:measure-h}}{\includegraphics[width=0.33\columnwidth]{eps/measure_height_bbox}}\hfill%
	% \subcaptionbox{Phone orientation animation\label{fig:orient}}{\includegraphics[width=0.5\columnwidth]{plot/rotate_phone}}
	\hfill%
	\subcaptionbox{Phone orientation effect (degree)\label{fig:measure-o}}{\includegraphics[width=0.325\columnwidth]{eps/measure_orientation_bbox}}\hfill%
	\hfill%
	\subcaptionbox{Temporal stability\label{fig:measure-t}}{\includegraphics[width=0.325\columnwidth]{eps/measure_temoral_bbox}}\hfill%

	\caption{Different affecting factors.}
	\label{fig:factors}
	%\vspace{-1em}
  \end{figure}

% $\blacksquare${\bf Scalability and resolution acoustic echoes}
% We use the fingerprinting-based approach to explore the spatial distinctness of acoustic echoes. Specifically, we evaluate the {\bf scalability} and the {\bf resolution} of the acoustic echoes used for location recognition. The {\bf scalability} refers to a research question that whether acoustic echo contains sufficient location information so that it can be used to recognize as many locations as possible. The {\bf resolution} refers to the spatial distinctness of the acoustic echoes. Intuitively, the acoustic echoes with small spatial distances will have similar patterns, thus a trained classifier may fail to discriminate such acoustic echoes.
  
  % We treat obtained echo spectrograms as 1-channel images and train a CNN for location classification. We adopt ResNet-18 architecture and customize the first layer to allow the a-channel spectrogram images as input. We implement the ResNet-18 using Pytorch.
%   $\blacksquare${\bf Data collection and model design}
  
\subsubsection{Localization resolution} 
  
To investigate the resolution of EchoPrint, we evaluate the EchoPrint's performance with respect to the spatial distance. We randomly select 12 locations with similar spatial distances, then train a DNN model and report the corresponding result. We change the spatial distance from $25 \text{cm}$ up to $300 \text{cm}$ and repeat the experiment 20 times for each distance. Fig. ~\ref{fig:eval-reso-acc} shows the recognition accuracy with respect to the spatial distance. There is no obvious trend when the spatial distance increases, indicating that EchoPrint is able to distinguish the echo differences even they are spatially close. Fig. ~\ref{fig:eval-reso-error} shows the mean recognition error with respect to the spatial distance. Similarly, there is no clear trend for recognition error when the spatial distance increases. EchoPrint can maintain a sub-meter recognition error {\red Need to add explaination}. In conclusion, EchoPrint can finely discriminate acoustic echoes that are spatially close. It is potentially used for fine-grained location recognition.
  
  %To address the training data scarcity of acoustic echoes and avoid extensive data collection by humans. We propose to augment the training data for CL by leveraging on the data produced by simulation tools. Note that a room's acoustic response is determined by various factors including its shape, wall materials, objects that occupy the room, material absorption and reflection rate, etc. The existing simulation tools are not yet able to generate accurate acoustic response to mimic a real room. We demonstrate this using an example. We employ pyroomacoustic \cite{scheibler2018pyroomacoustics} to construct a room with similar size to the demo room as shown in Fig.~\ref{fig:demo-room}. We use a 0.5 energy absorption for all walls. In simulation, we place a omni-diectional sound source at the center of the room and plays the deisigned logarithmic chirp. In addition, we mimic a smartphone recording by placing a microphone at 15$cm$ apart from the sound source to record the signal. We follow the same procedures in \sect\ref{subsec:chirp-design} to extract the spectrogram of the echo and compare it with a real spectrogram obtain from the same location in the real room. Fig.~\ref{fig:real-sim}a,~\ref{fig:real-sim}b show a comparison of simulated and real spectrogram. It is obvisously that the spectrograms are different in terms of the frequency energy distribution is time domain. 
	
  % Despite the acoustic features generated by simulation tool are different from a real room, the simualated acoustic features can be used for the purpose of contrastive feature representation learning. Fig.~\ref{fig:real-sim}b,~\ref{fig:real-sim}c show the spectrograms generated using $pyroomacoustic$ at two locations with 0.5$m$ apart. The generated features are spatially distinct, indicating that we can use the simulation to generate data for to augment the training dataset.  
  
  
  
%   $\blacksquare${\bf Performance Evaluation}
  
  We present the scalability and the resolution evaluation results, the metrics used are localization accuracy and the mean localization error. We also investigate the training data requirement for EchoPrint.
 % 31e_paper_plot_scalability_and_resoluation_line_boxplot
  \begin{figure}
	\begin{subfigure}[t]{.48\columnwidth}
	  \includegraphics[width=\columnwidth]{eps/eval_resolution_box}%{eps/conventional-da}
	  \caption{Resolution mean errors}
	  \label{fig:eval-reso-acc}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{.48\columnwidth}
		\includegraphics[width=\columnwidth]{eps/eval_scalability_box}%{eps/conventional-da}
		\caption{Scalability mean errors}
		\label{fig:eval-reso-error}
	  \end{subfigure}
	  %\vspace{-0.5em}
	\caption{Scalability and resolution evaluation}
	% \label{fig:tba}
	%\vspace{-2em}
\end{figure}
  % new
  \begin{comment}
  \begin{figure}
	  \begin{subfigure}[t]{.48\columnwidth}
		\includegraphics[width=\columnwidth]{eps/eval_resolution_accuracy}%{eps/conventional-da}
		\caption{Recognition accuray}
		\label{fig:eval-reso-acc}
	  \end{subfigure}
	  \hfill
	  \begin{subfigure}[t]{.48\columnwidth}
		  \includegraphics[width=\columnwidth]{eps/eval_resolution_error_mean}%{eps/conventional-da}
		  \caption{Recognition mean error}
		  \label{fig:eval-reso-error}
		\end{subfigure}
		%\vspace{-0.5em}
	  \caption{Resolution study}
	  % \label{fig:tba}
	  %\vspace{-2em}
  \end{figure}
  
  % 31e_paper_plot_scalability_and_resoluation_line_boxplot
  \begin{figure}
	  \begin{subfigure}[t]{.48\columnwidth}
		  \includegraphics[width=\columnwidth]{eps/eval_scalability_accuracy}
		  \caption{Recognition accuray}
		  \label{fig:eval-scale-acc}
	  \end{subfigure}
	  \hfill
	  \begin{subfigure}[t]{.48\columnwidth}
		\includegraphics[width=\columnwidth]{eps/eval_scalability_error_mean}
		\caption{Recognition mean error}
		\label{fig:eval-scale-error}
	  \end{subfigure}
	  %\vspace{-0.5em}
	  \caption{Scalability study.}
	  % \label{fig:tba}
	  %\vspace{-2em}
  \end{figure}
\end{comment}
  % \begin{figure}
  % 	\begin{subfigure}[t]{.48\columnwidth}
  % 	  \includegraphics[width=\columnwidth]{eps/eval_resolution_error_80pct_bp}%{eps/conventional-da}
  % 	  \caption{Resolution eval 80 percentile error}
  % 	  \label{fig:eval-reso-error}
  % 	\end{subfigure}
  % 	\hfill
  % 	\begin{subfigure}[t]{.48\columnwidth}
  % 	  \includegraphics[width=\columnwidth]{eps/eval_scalability_error_80pct_bp}
  % 	  \caption{Scalability eval 80 percentile error}
  % 	  \label{fig:eval-scale-error}
  % 	\end{subfigure}
  % 	%\vspace{-0.5em}
  % 	\caption{80 Percentile Error.}
  % 	% \label{fig:tba}
  % 	%\vspace{-2em}
  % \end{figure}
  
  % \begin{figure}
  % 	\begin{subfigure}[t]{.48\columnwidth}
  % 	  \includegraphics[width=\columnwidth]{eps/eval_resolution_error_85pct_bp}%{eps/conventional-da}
  % 	  \caption{Resolution eval 85 percentile error}
  % 	  \label{fig:eval-reso-error}
  % 	\end{subfigure}
  % 	\hfill
  % 	\begin{subfigure}[t]{.48\columnwidth}
  % 	  \includegraphics[width=\columnwidth]{eps/eval_scalability_error_85pct_bp}
  % 	  \caption{Scalability eval 85 percentile error}
  % 	  \label{fig:eval-scale-error}
  % 	\end{subfigure}
  % 	%\vspace{-0.5em}
  % 	\caption{85 Percentile Error.}
  % 	% \label{fig:tba}
  % 	%\vspace{-2em}
  % \end{figure}
  
  % \begin{figure}
  % 	\begin{subfigure}[t]{.48\columnwidth}
  % 	  \includegraphics[width=\columnwidth]{eps/eval_resolution_error_90pct_bp}%{eps/conventional-da}
  % 	  \caption{Resolution eval 90 percentile error}
  % 	  \label{fig:eval-reso-error}
  % 	\end{subfigure}
  % 	\hfill
  % 	\begin{subfigure}[t]{.48\columnwidth}
  % 	  \includegraphics[width=\columnwidth]{eps/eval_scalability_error_90pct_bp}
  % 	  \caption{Scalability eval 90 percentile error}
  % 	  \label{fig:eval-scale-error}
  % 	\end{subfigure}
  % 	%\vspace{-0.5em}
  % 	\caption{90 Percentile Error.}
  % 	% \label{fig:tba}
  % 	%\vspace{-2em}
  % \end{figure}
  
\subsubsection{Localization model scalability}
  To investigate the scalability of EchoPrint, we randomly select $K$ classes from 127 fingerprinted locations, then we train a DNN model with the selected dataset and report the corresponding result. We increase the class number $K$ from 10 to 120, and repeat the experiment 20 times for each $K$. Fig. ~\ref{fig:eval-scale-acc} shows the recognition accuracy with respect to the class numbers. It is observed that the recognition accuracy decreases when class number $K$ increases. The decreasing recognition accuracy trend is expected for DNN based model, as larger class numbers increase the feature space complexity. However, EchoPrint can maintain the recognition accuracy above 85\%. Fig. ~\ref{fig:eval-scale-error} shows the mean recognition error with respect to the class numbers. Similarly, the recognition error increases when the class number increases. EchoPrint can maintain a sub-meter recognition error. In conlusion, EchoPrint can be extended to a large scale and maintain a sub-meter recognition error in an indoor space.
  
  {\red (need to always tie to SLAM. What's the implication of the scalability result on SLAM? Is the decreasing trend in Fig. 8(b) and the increasing trend in Fig. 9(b) a disadvantage of the fingerprinting approach?)}
  
%   $\blacksquare${\bf Resolution of EchoPrint:}
  



% \subsubsection{Temporal stability of echoes}

\subsubsection{Stability of echos}

this section evaluates impact of user height, furniture change, ambient noise, etc

{\bf Sensitivity to user's height:} Users with different heights carry the smartphone at different heights. We study the acoustic features' sensitivity to the height in this experiment. We collect acoustic echoes from 70$cm$ to 100 $cm$, with a 10$cm$ difference at spot 2 of Fig. ~\ref{fig:demo-room}. We plot the power spectral density (PSD) of recorded echoes for different heights from 15kHz to 20kHz. Results are shown in Fig. ~\ref{fig:measure-h}. It's observed that PSDs at height 70$cm$ to 90$cm$ are similar with small differences. Whereas the PSD at 100$cm$ exhibit higher dissimilarity, implies that the acoustic signal can tolerate certain amount of height differences, ~20$cm$ {\red (need to argue that, when the user holds the phone in hand to do the localization, the height variations should be small)}.

{\bf Sensitivity to phone's orientation:} Phone orientation is a potential factor that influences the received acoustic feature at a spot. Echotag \cite{tung2015echotag} is able to discriminate the angle difference as small as $2^\circ$. We collect acoustic echoes by rotating the smartphone from $0^\circ$ to $180^\circ$, with a $45^\circ$ differences at spot 2 of Fig. ~\ref{fig:demo-room}. We plot the PSD of different angles and the results are shown in Fig. ~\ref{fig:measure-o}. It's observed that the PSDs from $0^\circ$ to $90^\circ$ exhibit high similarities whereas the PSDs from $135^\circ$ and $180^\circ$ are much different. This observation shows that the room's acoustic feature at certain location

{\bf Sensitivity to aging:}

\subsection{Summary}
{\red this subsec establishes the concept of "echoic location feature (ELF)}
% Impact of moving people

% Impact of changed furniture

% Impact of ambient noise, % {\red TODO including the effect of co-existance of probing chirps}

% Impact of room size

% $\blacksquare${\bf How much training data is needed?:}
% {\red (this graph not ready yet)}Albeit achieves sub-meter location recognition errors, a DNN-based model requires substantial training data. We plot Fig.~\ref{fig:dnn-acc} to characterize the DNN's performance against the volume of training data. Horizontal axis represents the training data available for each location, vertical axis represent the DNN localization accuracy on test dataset. It's expected that DNN's performance increases with more training data available for each class. We observe that DNN's performance saturated when number of training data in each class larger than 1500, representing 5 hours' training data collection time. Although it is one-time effort, long training data collection time still impede the applicability of DNN-based approach. 

% The research question is, how can we reduce the training data collection effort whereas maintain the performance of DNN for localization?


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


% \subsection{Training data reduction with CL}


% \begin{figure}
% 	\begin{subfigure}[t]{.45\columnwidth}
% 	  \includegraphics[width=\columnwidth]{eps/cdnn_acc_vs_data_volumn}%{eps/conventional-da}
% 	  \caption{Model accuracy vs data volumn}
% 	  \label{fig:dnn-acc}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[t]{.45\columnwidth}
% 	  \includegraphics[width=\columnwidth]{eps/cdnn_acc_vs_data_volumn}
% 	  \caption{TBA}
% 	  \label{fig:tba}
% 	\end{subfigure}
% 	%\vspace{-0.5em}
% 	\caption{TBA.}
% 	% \label{fig:tba}
% 	%\vspace{-2em}
%   \end{figure}

% \subsubsection{Feature distinctness of CL}

% \begin{figure}
% 	% \vspace{1em}
% 	\subcaptionbox{Spectrogram\label{fig:cos-ori}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_cosine_original}}\hfill%
% 	\subcaptionbox{tSNE feature\label{fig:cos-tsne}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_cosine_tsne}}\hfill%
% 	%\subcaptionbox{SimCLR\label{fig:cos-cl0}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_simclr_cosine_cl.eps}}\hfill%
% 	\subcaptionbox{SupCon baseline\label{fig:cos-cl1}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_supcon_cosine_cl}}\hfill%
% 	\subcaptionbox{SupCon proposed\label{fig:cos-cl2}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_supconHard_cosine_cl}}\hfill%
% 	\subcaptionbox{Spectrogram\label{fig:euc-ori}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_euclidean_original}}\hfill%
% 	\subcaptionbox{tSNE feature\label{fig:euc-tsne}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_euclidean_tsne}}\hfill%
% 	%\subcaptionbox{SimCLR\label{fig:euc-cl0}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_simclr_euclidean_cl}}\hfill%
% 	\subcaptionbox{SupCon baseline\label{fig:euc-cl1}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_supcon_euclidean_cl}}\hfill%
% 	\subcaptionbox{SupCon proposed\label{fig:euc-cl2}}{\includegraphics[width=0.25\columnwidth]{eps/pdf_supconHard_euclidean_cl}}\hfill%

% 	\caption{Distribution of Euclidean/Cosine distance between acoustic features at same or different locations. {\red These figures drawn using simul+real pretrained model}}
% 	\label{fig:feat-dist}
% 	%\vspace{-1em}
%   \end{figure}



% {\red hint: same spots while with moving people}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> tips.tex <==
\section{Latex Tips}
\label{sec:tip}

\subsection{insert circled number}
\ding{182} One \ding{183} two

\subsection{Underline}
\underline{Th}is is how to do it

\subsection{Emphasis}
{\em this is how to do it}

\subsection{Highlight}
{\red this is how to do it}

\subsection{Citation}
This is citation \cite{tiku2020hidden}

\subsection{BlackSquare}
$\blacksquare$ This is how to do it


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

